On optimum left-to-right strategies for active context-free games

Active context-free games are two-player games on strings over finite alphabets with one player trying to rewrite the input string to match a target specification. These games have been investigated in the context of exchanging Active XML (AXML) data. While it was known that the rewriting problem is undecidable in general, it is shown here that it is EXPSPACE-complete to decide for a given context-free game, whether all safely rewritable strings can be safely rewritten in a left-to-right manner, a problem that was previously considered by Abiteboul et al. Furthermore, it is shown that the corresponding problem for games with finite replacement languages is EXPTIME-complete.

==> abstract.tex <==
\emph{Active context-free games} are two-player games on strings over finite alphabets with one player trying to rewrite the input string to match a target specification. These games have been investigated in the context of exchanging Active XML (AXML) data. While it was known that the rewriting problem is undecidable in general, it is shown here that it is $\EXPSPACE$-complete to decide for a given context-free game, whether all safely rewritable strings can be safely rewritten in a \emph{left-to-right} manner, a problem that was previously considered by Abiteboul et al. Furthermore, it is shown that the corresponding problem for games with finite replacement languages is $\EXPTIME$-complete.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 

==> conclusion.tex <==
\section{Conclusion}

We investigated a practically relevant restriction of strategies for context-free games and their relation to general strategies.  That $\lrall$ is $\EXPSPACE$-complete in general but $\EXPTIME$-complete in the restricted case where the replacement languages in $G$ are finite, is somewhat surprising, since the word problem of checking whether a given string is safely rewritable in a left-to-right fashion is $\EXPTIME$-complete in both cases\cite{MuschollSS06}.

The automaton construction for $\safelr$ we give here can be generalised to yield automata for strings which can be safely rewritten using up to $k$ left steps (with a full L2R pass being played before each left step). This is done by generalising our definition of effects to \emph{$k$-effects}, each of which is a set of sets of $(k-1)$-effects representing games on later passes. In this framework, effects as defined in this paper would correspond to $1$-effects.

It can also be shown that for every game $G$ there is a game $G'$ with finite replacement languages whose safely rewritable strings are exactly those of $G$. 

A further open frontier remains in the form of \emph{One-Pass} (1P) strategies~\cite{AbiteboulMB05}, which restrict L2R strategies by forcing \pone to make her decisions in a streaming manner, i.e. without knowing the entire input string. While Abiteboul, Milo and Benjelloun \cite{AbiteboulMB05} have shown a number of interesting properties of such strategies, the general problem of testing whether every safely L2R-rewritable string of a given game can also safely rewritten in a 1P fashion is not even known to be decidable.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 
